A logic for n-dimensional hierarchical refinement

Hierarchical transition systems provide a popular mathematical structure to represent state-based software applications in which different layers of abstraction are represented by inter-related state machines. The decomposition of high level states into inner sub-states, and of their transitions into inner sub-transitions is common refinement procedure adopted in a number of specification formalisms. This paper introduces a hybrid modal logic for k-layered transition systems, its first-order standard translation, a notion of bisimulation, and a modal invariance result. Layered and hierarchical notions of refinement are also discussed in this setting.

==> eptcsdata.tex <==
\providecommand{\firstpage}{40}
\providecommand{\publicationstatus}{Eerke Boiten, John Derrick \& Steve Reeves (Eds.):\\
Refinement Workshop 2015 (Refine '15)\\
EPTCS 209, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.209.4}{10.4204/EPTCS.209.4}}
\pdfoutput=1

